Data-driven bandwidth choice for gamma kernel estimates of density derivatives on the positive semi-axis

In some applications it is necessary to estimate derivatives of probability densities defined on the positive semi-axis. The quality of nonparametric estimates of the probability densities and their derivatives are strongly influenced by smoothing parameters (bandwidths). In this paper an expression for the optimal smoothing parameter of the gamma kernel estimate of the density derivative is obtained. For this parameter data-driven estimates based on methods called "rule of thumb" and "cross-validation" are constructed. The quality of the estimates is verified and demonstrated on examples of density derivatives generated by Maxwell and Weibull distributions.

==> reference.tex <==
@InProceedings{Bonald,
author = {T. Bonald and L. Massouli\'{e} and F. Mathieu and D. Perino and A. Twigg},
title = {Epidemic Live Streaming: Optimal Performance Trade-Offs},
booktitle = {Proc. of ACM SIGMETRICS 2008},
OPTcrossref = {},
OPTkey = {},
pages = {325-336},
year = {2008},
OPTeditor = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTmonth = {},
OPTorganization = {},
OPTpublisher = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}



%\bibitem{Wang}
%Wang K., Jiang Y., Lin C.: Modeling and Analysis of a P2P-VoD System Based on Stochastic Network Calculus. In: Measurement, Modelling, and Evaluation %of Computing Systems and Dependability and Fault Tolerance,  ISBN 978-3-642-28539-4, Series: Lecture Notes in Computer Science 7201, 302-316, %Springer, 2012

